EFCNet: Every Feature Counts for Small Medical Object Segmentation

This paper explores the segmentation of very small medical objects with significant clinical value. While Convolutional Neural Networks (CNNs), particularly UNet-like models, and recent Transformers have shown substantial progress in image segmentation, our empirical findings reveal their poor performance in segmenting the small medical objects and lesions concerned in this paper. This limitation may be attributed to information loss during their encoding and decoding process. In response to this challenge, we propose a novel model named EFCNet for small object segmentation in medical images. Our model incorporates two modules: the Cross-Stage Axial Attention Module (CSAA) and the Multi-Precision Supervision Module (MPS). These modules address information loss during encoding and decoding procedures, respectively. Specifically, CSAA integrates features from all stages of the encoder to adaptively learn suitable information needed in different decoding stages, thereby reducing information loss in the encoder. On the other hand, MPS introduces a novel multi-precision supervision mechanism to the decoder. This mechanism prioritizes attention to low-resolution features in the initial stages of the decoder, mitigating information loss caused by subsequent convolution and sampling processes and enhancing the model's global perception. We evaluate our model on two benchmark medical image datasets. The results demonstrate that EFCNet significantly outperforms previous segmentation methods designed for both medical and normal images.

==> sec/0_abstract.tex <==
\begin{abstract}
\iffalse
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\fi

Convolutional neural networks (CNNs), specifically UNet-like models have made great progress in the field of medical image segmentation. However, these models cannot handle the information loss during the auto-encoding process. As a result, they generally perform poorly on small objects and lesions, which are extremely common in medical research, thus making them impractical. To solve this problem, we propose a novel autoencoder named as EFCNet for small object segmentation in medical images. Our model contains two modules named Cross-Stage Axial Attention Module (CSAA) and Multi-Precision Supervision Module (MPS) that solve the information loss during encoding and decoding procedures respectively. Specifically, CSAA integrates features in all stages of the encoder so as to adaptively learn suitable information required in different decoding stages, thus reducing the loss of information in the encoder. On the other hand, MPS adds a novel multi-precision supervision mechanism to the decoder, which pays sufficient attention to low-resolution features in the first few stages of the decoder, thereby alleviating the problem of information loss caused by the subsequent convolution and sampling process, and improving model's ability of global perception. We evaluate our model on two benchmark medical image datasets, whose result demonstrates that EFCNet can significantly outperform previous segmentation methods that are designed for both medical and normal images.

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Small medical objects are common in disease research, such as HyperReflective Dots (HRDs) on Optical Coherence Tomography (OCT). Studies have proved that these small lesions are of great significance to medical diagnosis and treatment \cite{qin2021hyperreflective,huang2021algorithm,arthi2021hyperreflective,chung2019role}. However, manually labeling small objects in these medical images is time-consuming and labor-intensive, which is a great waste of medical resources. Therefore, there is a great need to automatically segment small medical objects with the help of AI algorithms. Fortunately, with the rapid development of deep learning methods, many Convolution neural networks (CNNs) have been proposed for medical image segmentation, such as U-Net \cite{ronneberger2015u}, ResUNet \cite{8589312}, DenseUNet \cite{8697107}, ResUNet++ \cite{jha2019resunet} and MultiResUNet \cite{ibtehaz2020multiresunet}. 

However, there are few studies dedicated to segmentation of small medical objects which are common in medical research. Moreover, we find that the previous segmentation methods 
 generally suffer from information loss, which can be stated as the following two points: (1) The previous methods \cite{ronneberger2015u,jha2020doubleu} generally adopt features from the previous stage and the corresponding stage in the encoder through the lateral connections. This means only limited levels of features are directly utilized for each decoding stage, which conflicts with the previous studies \cite{poudel2018contextnet,cheng2020cascadepsp} that show both shallow features and deep features can help improve the accuracy of segmentation. Various types of information in other stages in the encoder are not directly utilized. This pattern results in a huge loss of information in the encoder. (2) Most of the previous methods \cite{8589312,jha2020doubleu,huang2020unet} only add one segmentation head for supervision at the last stage of the decoder. Some studies \cite{zhang2018exfuse,chen2014semantic,chen2017deeplab} have shown that the low-resolution features in the first few decoding stages have strong global perception , thus being informative for the localization of small objects. However, the information contained in the these stages of the decoder is lost to some extent during the convolution and upsampling process. 
 
\begin{figure*}
    \centering
    \includegraphics[width=13cm]{intro_final.pdf}
    \caption{Comparison of our method against SAM on two medical image datasets of small objects.}
    \label{in_fig}
\end{figure*}

Compared with objects of normal size, small medical objects contain less information, which means that information loss of a model will have a more serious impact on the segmentation accuracy. And this is a typical segmentation task that the SAM model~\cite{kirillov2023segment} does not work well as in Fig.~\ref{in_fig}. %Therefore the information loss caused by the previous methods has a great negative impact on small medical object segmentation.

To alleviate the problem of information loss during segmentation, we propose a novel solution, which is based on the autoencoder structure. Our model pays enough attention to all the features in each stage of both encoder and decoder, thereby improving the accuracy of small object segmentation. Concretely, for the encoder, we proposed the Cross-Stage Axial Attention Module (CSAA), which use the attention mechanism to integrate all the features of all stages in the encoder, so that the model can adaptively learn information needed for each decoding stage. Through CSAA, the decoding process of each stage in the decoder can directly refer to all useful information in the encoder, thereby alleviating the information loss of the encoder. Meanwhile, we propose the Multi-Precision Supervision Module (MPS) for the decoder, which adds segmentation heads with different precision for supervision after each stage in the decoder. Low-precision segmentation heads are utilized for low-resolution features in order to temporarily ignore the pursuit of local details and give full play to the advantages of its strong global perception. With the help of MPS, the model can sufficiently exploit information contained in the features of each stage in the decoder, thereby alleviating the information loss in the decoder.

To validate the efficacy of the proposed method, we conduct extensive experiments on two datasets, including a fundus Optical Coherence Tomography (OCT) image dataset constructed by us and a subdataset from CVC-ClinicDB \cite{bernal2015wm}. Experimental results on these two datasets demonstrate that our method outperforms previous state-of-the-art models in terms of dice similarity coefficient (DSC) and intersection over union (IoU).

Our contributions can be summarized as follows: \\
1. We propose a novel idea to face the challenge of small medical object segmentation. We believe that every feature counts for small object segmentation in medical images. Our model pays attention to all features of each stage in the model and mines various information contained in them, thereby reducing information loss of small medical objects. \\
2. We design two modules named Cross-Stage Axial Attention Module (CSAA) and Multi-Precision Supervision Module (MPS), to effectively reduce the information loss in the encoder and decoder respectively and therefore improve segmentation accuracy of the model. \\
3. We construct a new benchmark for the study of small medical objects segmentation. And our experiments on two datasets of small medical objects demonstrate that our model outperforms the previous state-of-the-art models to a large extent.



==> sec/2_related.tex <==
\section{Related Works}
\noindent \textbf{Medical Image Segmentation}
Recently, various innovative methods \cite{chen2018drinet,milletari2016v,gu2019net,hatamizadeh2022unetr,valanarasu2022unext} have been proposed for semantic segmentation in medical images. Zhang et al. \cite{zhang2021transfuse} proposed a novel hybrid structure that combines CNN and Transformer in parallel, which reduced the loss of low-level details. Chen et al. \cite{chen2021transunet} embedded Transformer module into the encoder of U-Net, which improved the long-range modeling ability of the model. Wang et al. \cite{wang2022stepwise} used a Transformer encoder to alleviated the overfitting phenomenon, and designed Progressive Locality Decoder to enhance local information of medical images. Although these methods above have played a great role in medical image segmentation, they have not fully considered the impact of object size on segmentation results. These models tend to perform poorly when faced with small object segmentation. Lou et al. \cite{lou2022caranet} considered the impact of medical object size on segmentation process and proposed an Context Axial Reverse Attention module (CaraNet) to help the model detect local information of small medical objects. However, bilinear interpolation used in the decode stage of CaraNet will cause serious information loss, which has a great negative impact on small medical object segmentation. Different from methods mentioned above, our model reduces the information loss of small medical objects through CSAA and MPS, and thus effectively improves the segmentation accuracy.

\noindent \textbf{General Segmentation Model}
Recently, Kirillov et al.~\cite{kirillov2023segment} proposed a Segment Anything Model (SAM), a general segmentation model which has made important progress in natural image segmentation. However, due to the fine structures and complex boundaries in medical images, SAM is not suitable for most medical image segmentation tasks, including small object segmentation, without manual guidance \cite{huang2023segment,he2023accuracy}.

\noindent \textbf{Attention Mechanism}
Plenty of Attention-based methods \cite{oktay2018attention,shen2018reinforced,huang2019attention,sinha2020multi,tao2020hierarchical} have been proposed in recent years for various tasks in computer vision and natural language processing. Vaswani et al. \cite{vaswani2017attention} abandoned the traditional convolutional structure and  constructed a novel architecture named Transformer using attention mechanisms. Woo et al. \cite{woo2018cbam} added both Channel Attention and Spatial Attention in convolutional neural networks. Zhang et al. \cite{zhang2022epsanet} proposed the Pyramid Squeeze Attention Module (PSA) to help the model explore spatial information at different scales. Inspired by the attention-baseds method mentioned above, we propose Cross-Stage Axial Attention Module (CSAA), which facilitates the feature fusion and reduces information loss in the model.

==> sec/3_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_method.tex <==
\section{Method}
% In this chapter, we first introduce the task of small medical object segmentation and some notations in Section~\ref{setup}. Next, we introduce the overall structure of EFCNet in Section~\ref{overall}. Then, we show the details of Cross-Stage Axial Attention Module (CSAA) and Multi-Precision Supervision Module (MPS) in Section~\ref{CSAA} and Section~\ref{MPS}, respectively. Finally, we introduce the Loss Function of our model in Section~\ref{loss}.
We begin by introducing the task of small medical object segmentation and related notations. Then, we present the overall structure of EFCNet (Sec.~\ref{overall}) and explain the specifics of the Cross-Stage Axial Attention Module (CSAA) and the Multi-Precision Supervision Module (MPS) in Sec.~\ref{CSAA} and Sec.~\ref{MPS} respectively. Finally, we discuss the Loss Function of our model (Sec.~\ref{loss}).

%\paragraph{Problem setup and notations}
\noindent \textbf{Problem Setup and Notations}.
%\label{setup}
In our segmentation task, we denote the medical picture dataset as $X = \{x_{1}, ..., x_{n} | x_{i} \in R^{C\times H\times W} \} $. Lesions in each image \(x_{i}\) are carefully and manually annotated by doctors, constituting the ground truth set $Y = \{y_{1}, ..., y_{n} | y_{i} \in \{0,1\}^{1\times H\times W} \} $. We denote the total dataset as \(D=\{X, Y\}\). \(D\) is usually divided into training set $ D_{train}=\{X_{train}, Y_{train}\}$ and testing set $D_{test} = \{X_{test}\}$. 

Our task is to design an algorithm so that our model can learn the ability to segment small medical objects from \(D_{train}\) and perform well in \(D_{test}\).


\subsection{Overall Architecture}
\label{overall}

\begin{figure*}
    \centering
    \includegraphics[width=13cm]{overview_final.pdf}
    \caption{Overview of our EFCNet, which contains a U-Net architecture with CSAA module and MPS module.}
    \label{all_fig}
\end{figure*}

As shown in Fig.~\ref{all_fig}, a medical image 
containing small object lesions is fed into our model as input. First, the image passes through the encoder with \(K\) stages, obtaining feature maps containing various types of information of small medical objects. Next, features in all stages of the encoder are put into CSAA Module, forcing the model to adaptively learn information about small medical objects that is conducive to the decoding procedure. Then, the decoder processes the feature maps stage by stage under the guidance of CSAA Module. Finally, feature maps of all stages in the decoder are put into MPS Module to obtain multi-precision prediction results and get supervisions separately. In the testing phase, we use the output of the last stage of decoder as the final segmentation result of our model.

\subsection{CSAA Module}
\label{CSAA}

\begin{figure*}
    \centering
    \includegraphics[width=14cm]{csaa_final.pdf}
    \caption{Structure of CSAA module, which fuses all features in each stage of the encoder, extracts the information about small medical objects adaptively, and guides the decoding process of each stage in the decoder.}
    \label{csaa_fig}
\end{figure*}

Features in different stages of the encoder contain different kinds of information about small medical objects. However, most of the information cannot be directly used by the decoder, and some information is even lost in the convolution and downsampling process. In order to reduce the information loss in the encoder, we design Cross-Stage Axial Attention Module (CSAA), which adaptively learns information from features in all stages of the encoder, and then guides the subsequent decoding work. As shown in Fig.~\ref{csaa_fig}, CSAA includes three steps: reshaping, axial-attention and compressing. 

\noindent \textbf{Reshaping}.
To facilitate the fusion of features in all stages of the encoder, we adjust the size of all feature maps in each stage of the encoder to the same size as the feature map in the corresponding decoding stage \(j\) in both spatial and channel dimension, through convolution operations. 
\begin{equation}
    \begin{split}
        &f_{i,j}^{*} = \sigma (BN(conv_{j}^{Reshape}(f_{i}^{e}))) \\& \in \mathbb R^{C_{j} \times H_{j} \times W_{j}}, i,j=1,2,..,K
    \end{split}  
\end{equation}
where \(f_{i}^{e}\) represents the feature map in stage \(i\) of the encoder. \(K\) is the number of stages in the encoder and decoder. \(\sigma\) and \(BN\) denote ReLU and Batch Normalization respectively. 
Then we concatenate all resized features \(\{f_{i,j}^{*}\}_{i=1}^{K}\) in channel dimension to obtain a new feature \(f_{j}^{*}\) with a size of \((KC_{j}, H_{j}, W_{j})\), which is regarded as the input of next step: Axial-Attention.
\begin{equation}
    \begin{split}
        &f_{j}^{*} = Concat(f_{1,j}^{*},f_{2,j}^{*},...,f_{K,j}^{*}) \\& \in \mathbb R^{KC_{j} \times H_{j} \times W_{j}}, j=1,2,..,K
    \end{split}
\end{equation}

\noindent \textbf{Axial-Attention}.
We put \(f_{j}^{*}\) into an axial attention model \cite{huang2019ccnet} working on two spatial dimensions \(H\) and \(W\), in order to comprehensively learn information of all feature maps processed from the encoder, and thus adaptively guide the decoding process of each stage in the decoder.
\begin{equation}
    \begin{split}
        &f_{j}^{Attn} = SA_{W}(SA_{H}(f_{j}^{*})) \\& \in \mathbb R^{KC_{j} \times H_{j} \times W_{j}}, j=1,2,..,K
    \end{split}
\end{equation}
where \(SA_{W}\) and \(SA_{H}\) represent axial attention on width dimension and height dimension respectively. It is worth mentioning that considering that conventional two-dimensional self-attention consumes a lot of computing resources\cite{wang2020axial}, we adopt a two-stage one-dimensional self-attention model here, performing self-attention processing on the feature maps in the Height and Width dimensions in turn.

\noindent \textbf{Compressing}.
In order to facilitate the guidance to decoding procedure with the information obtained by axial attention, \(f_{j}^{Attn}\) is compressed to the same size as the feature map of the corresponding stage in the decoder, through convolution operations.

\begin{equation}
    \begin{split}
        &f_{j}^{Comp} = \sigma (BN(conv_{j}^{Comp}(f_{j}^{Attn}))) \\ &\in \mathbb R^{C_{j} \times H_{j} \times W_{j}}, j=1,2,..,K 
    \end{split}   
\end{equation}

where \(\sigma\) and \(BN\) denote ReLU and Batch Normalization respectively. At the end of CSAA, we concatenate \(f_{j}^{Comp}\) to the feature map of the corresponding stage in the decoder in channel dimension.

As can be seen, CSAA helps the model mine the  information about small medical objects in the encoder to a great extent, and assigns it to the corresponding stage of the decoder.Different from previous models, our decoding procedure of each stage in the decoder is guided by segmentation related information exploited from all stages of the encoder, with the help of CSAA. Through CSAA, our model realizes feature fusion in encoder, strengthens the connection between encoder and decoder, and reduces the loss of information in encoder to a large extent.



%We take stage2 as an example to show the working details of CSAA, as shown in Figure~\ref{csaa_fig}. First, we adjust the size of all feature maps in four stages of the encoder to the same size as that of stage2, i.e. \( (2\times C, \frac{H}{2}, \frac{W}{2}) \), through convolution and deconvolution operations.

%Next, we concatenate all resized features of the encoder in channel dimension to obtain a new feature \(feature_{all}\) with a size of \( (8\times C, \frac{H}{2}, \frac{W}{2}) \). Then, we put \(feature_{all}\) into an axial attention model to comprehensively consider all feature maps of each channel, and thus adaptively obtain corresponding useful information to guide the decoding process of each stage in the decoder. It is worth mentioning that considering that conventional two-dimensional self-attention consumes a lot of computing resources, we adopt a two-stage one-dimensional self-attention model here, performing self-attention processing on the feature maps in the H and W dimensions, respectively. Finally, the output of axial attention model is adjusted to the same size as that of stage2, i.e. \( (2\times C, \frac{H}{2}, \frac{W}{2}) \), through simple convolution operation, and is regarded as the final output of CSAA, which is concatenated into the corresponding stage of the decoder.

\subsection{MPS Module}
\label{MPS}

\begin{figure*}
    \centering
    \includegraphics[width=14cm,height=6cm]{mps_final.pdf}
    \caption{Structure of MPS module, which outputs segmentation predictions of different precision, and supervises them by the ground truth.}
    \label{mps_fig}
\end{figure*}

Low-resolution features in the decoder have strong global perception, which can help the model improve performance on small medical object segmentation. In previous models ~\cite{ronneberger2015u,chen2021transunet,lou2022caranet}, however, the globally perceptual information is not fully exploited, and much of the useful information is lost in subsequent convolution and upsampling process. In order to solve this problem, we design Multi-Precision Supervision Module (MPS) to mine the information of low-resolution features in the decoder and reduce its loss in subsequent decoding process. As shown in Fig.~\ref{mps_fig}, MPS includes two steps: segmentation and upsampling.

\noindent \textbf{Segmentation}.
In order to mine the information of small medical object contained in each stage of the decoder adequately, we sent feature maps in each stage of the decoder to corresponding segmentation heads separately, and thus we get segmentation results with different resolutions \(\{P_{i}\}_{i=1}^K\).
\begin{equation}
   P_{i} = S(\sigma (BN(conv_{i}^{pred}(f_{i}^{d})))), i=1,2,..,K 
\end{equation}
where \(f_{i}^{d}\) represents the feature map in stage \(i\) of the decoder. \(\sigma\) and \(BN\) denote ReLU and Batch Normalization respectively. \(S(.)\) represents the sigmoid function.

\noindent \textbf{Upsampling}.
We use  neighbor interpolation method to upsample the segmentation results obtained in the previous step to the size same as the ground truth image, and therefore we get multi-precision segmentation for small medical objects. 
\begin{equation}
   M_{i} = Upsample(P_{i}), i=1,2,..,K
\end{equation}
We supervise the segmentation results of different precision with the ground truth label, to ensure that each stage of the decoder contains enough information to support the segmentation of small medical objects.

As mentioned above, we design supervision modes with different precision for features of different resolutions. Considering that low-resolution features have strong global perception but lack local details, we use low-precision supervision for them in order to temporarily give up the pursuit of local details but give full play to the advantages of low-resolution features with strong global perception. This multi-precision supervision approach preserves the advantages of the traditional single-segmentation head while retaining more global perception from low-resolution features for the model, thereby improving the performance on small medical objects segmentation.

\subsection{Loss function}
\label{loss}
Considering that the positive and negative pixels are extremely unbalanced in small medical object segmentation tasks, we use a combination of DiceLoss \cite{sudre2017generalised} and Binary Cross Entropy(BCE) Loss during the training process. For the segmentation map output by each stage of the decoder, we set the loss as:
\begin{equation}
    \begin{split}
        &L_{i} = \lambda_{1}\cdot L_{Dice} (M_{i}, Y) + \lambda_{2}\cdot L_{BCE} (M_{i}, Y), \\& i=1,2,..,K
    \end{split}
\end{equation}

where \(M_{i}\) represents the result predicted by the model at stage \(i\), and \(Y\) represents the ground truth. \(\lambda_{1}\) and \(\lambda_{2}\) are hyperparameters used to balance DiceLoss and BCELoss.
%We set \(\lambda_{1}=0.7\) and \(\lambda_{2}=0.3\) in the experiments.
Taking into account all segmentation results output by each stage of the decoder, the total loss of the model is
\begin{equation}
    L_{total} = \sum_{i=1}^K\alpha_{i}\cdot L_{i} 
\end{equation}
where  hyperparameter \(\{\alpha _{i}\}_{i=1}^{K}\) leverage losses of segmentation results with different precision.
%We set \(alpha_{1}\), \(alpha_{2}\), \(alpha_{3}\), \(alpha_{4}\) to 0.7, 0.8, 0.9, 1.0 respectively in the experiments.


==> sec/4_exp.tex <==
\section{Experiment}

\begin{figure*}
    \centering
    \includegraphics[width=14cm]{eg_final.pdf}
    \caption{Samples of small lesions in S-HRD and S-Polyp.}
    \label{v_explan}
\end{figure*}

%\noindent \textbf{Experimental Setup}.
\noindent \textbf{S-HRD Dataset}.
We collect 313 optical coherence tomography (OCT) images of macular edema patients and aim to segment the small HyperReflective Dots (small HRDs) in them. The dataset is dubbed as S-HRD, and S is for 'Small'. In S-HRD, the area of each lesion is less than 1 percent of the size of an entire image. We confirm that appropriate consent has been obtained for the use and display of images in our research. And we are fully prepared to make the dataset publicly available. More details of data collection process and privacy concerns are introduced in Sec. xxx? of Supplementary Material.

\noindent \textbf{S-Polyp Dataset}.
We select a polyp segmentation dataset CVC-ClinicDB \cite{bernal2015wm}, delete images containing large medical lesions, and keep 229 images in which all lesions are small medical objects. We name this dataset S-Polyp. The area of each lesion is less than 5 percent of the size of an entire image. Some examples of S-HRD and S-Polyp are shown in Fig.~\ref{v_explan}.

In order to avoid limitation and particularity of the two datasets, we use five-fold cross-validation to evaluate the performance of our model. 

\noindent \textbf{Definition of Small Objects}. Since there is no uniform definition of small medical objects in previous works, we define it in our work: If the ratio of the number of pixels \(n\) in an object to the number of pixels \(N\) in the entire picture is less than 5\(\%\), then the object is called a small medical object. If the ratio is less than 1\(\%\), we call the object an extremely small medical object. In S-Polyp, all objects are small medical objects. In S-HRD, all objects are extremely small medical object.

\noindent \textbf{Evaluation Metrics}.
We use two common metrics to compare our model with previous state-of-the-art models.
Dice Similariy Coefficient (DSC): DSC is defined as:
\begin{equation}
    DSC =\frac{2 \times |P\cap G|}{|P|+|G|} 
\end{equation}

where \(P\) represents the area of the predicted label and \(G\) represents the  area of the ground truth.
Intersection over Union (IoU): IoU is defined as:
\begin{equation}
    IoU =\frac{S_{i}}{S_{u}} 
\end{equation}

where \(S_{i}\) represents the area where the predicted label and the ground truth overlap, and \(S_{u}\) represents the total area of the two.

\noindent \textbf{Implementation Details}.
Our experiments are implemented on an NVIDIA RTX A6000 GPU with 48GB of memory. We use the SGD optimizer with an initial learning rate of 0.01. Our training process lasts for 200 epochs with a batch size of 4. All input images are uniformly resized to 352\(\times\)352. The number of stages in encoder and decoder of our model is set to 4. 

\noindent \textbf{Competitors}.
Since there are few works specially dedicated to small medical object segmentation, we choose recent models in the field of medical image segmentation as a reference, including state-of-the-art models: (1) CNN based methods: U-Net \cite{ronneberger2015u},Attention-UNet \cite{oktay2018attention},MSU-Net \cite{su2021msu}, CaraNet \cite{lou2022caranet}; (2) Transformer based methods: TransFuse \cite{zhang2021transfuse}, TransUNet \cite{chen2021transunet}, SSFormer \cite{wang2022stepwise}, Swin-UNet \cite{cao2022swin}; (3) Segment Anything Model (SAM) \cite{kirillov2023segment} and the related works: SAM without any prompt, SAM with point, SAM with box and MedSAM \cite{ma2023segment}. (4) We alse test the performance of the enlarged version of U-Net (U-Net-Large), which are simply scaled up from 4 layers to 12 layers, in order to explore the influence of model size on segmentation accuracy.


\subsection{Quantitative Results}
\begin{table} \small
  \caption{Comparison of our EFCNet with competitors on S-HRD and S-Polyp in DSC ($\%$) and IoU ($\%$).}
  \label{all_hrd}
  \centering
 \tabcolsep=0.05cm
  \begin{tabular}{cccccccc}
    \toprule
    Metrics & Methods & Fold0 & Fold1 & Fold2 & Fold3 & Fold4 & Mean \\
    \midrule
    \multirow{14}*{DSC ($\%$)} 
    & U-Net ~\cite{ronneberger2015u} & 42.09 & 36.51 & 37.74 & 35.90 & 41.29 & 38.71\\
    & U-Net-Large ~\cite{ronneberger2015u} & 43.02 & 36.72 & 38.24 & 37.82 & 41.60 & 39.48\\
    & Attn-UNet ~\cite{oktay2018attention} & 44.14 & 39.79 & 38.76 & 38.24 & 39.80 & 40.15\\
    & MSU-Net ~\cite{su2021msu} & 45.08 & 41.97 & 39.64 & 39.51 & 40.44 & 41.33\\
    & CaraNet ~\cite{lou2022caranet} & 17.03 & 13.79 & 12.46 & 13.40 & 13.07 & 13.95\\
    & TransUNet ~\cite{chen2021transunet} & 32.84 & 30.34 & 30.71 & 31.54 & 32.81 & 31.65\\
    & TransFuse ~\cite{zhang2021transfuse} & 14.95 & 10.11 & 11.59 & 11.96 & 11.13 & 11.95\\
    & SSFormer ~\cite{wang2022stepwise} & 34.66 & 27.74 & 27.06 & 28.49 & 25.97 & 28.78\\
    & Swin-UNet ~\cite{cao2022swin} & 07.90 & 04.27 & 04.29 & 08.08 & 07.32 & 06.37\\
    & SAM ~\cite{kirillov2023segment} & 03.81 & 03.66 & 01.47 & 01.40 & 02.89 & 02.64\\
    & SAM (box) ~\cite{kirillov2023segment} & 03.99 & 02.78 & 02.60 & 02.67 & 02.55 & 02.92\\
    & SAM (point) ~\cite{kirillov2023segment} & 10.49 & 07.48 & 05.16 & 04.66 & 07.79 & 07.12\\
    & MedSAM ~\cite{ma2023segment} & 04.07 & 03.29 & 03.16 & 02.86 & 03.11 & 03.30\\
    & \textbf{EFCNet(Ours)} & \textbf{49.10} & \textbf{44.91} & \textbf{43.72} & \textbf{43.46} & \textbf{44.95} & \textbf{45.23}\\
    \midrule
    \multirow{14}*{IoU ($\%$)} 
    & U-Net ~\cite{ronneberger2015u} & 28.83 & 24.09 & 24.20 & 24.12 & 26.90 & 25.63\\
    & U-Net-Large ~\cite{ronneberger2015u} & 29.99 & 25.21 & 25.13 & 25.09 & 27.88 & 26.66\\
    & Attn-UNet ~\cite{oktay2018attention} & 30.75 & 27.47 & 26.27 & 25.95 & 26.68 & 27.42\\
    & MSU-Net ~\cite{su2021msu} & 31.18 & 28.96 & 26.58 & 26.46 & 26.74 & 27.98\\
    & CaraNet ~\cite{lou2022caranet} & 10.36 & 08.04 & 07.21 & 07.77 & 07.50 & 08.18\\
    & TransUNet ~\cite{chen2021transunet} & 22.00 & 19.87 & 19.55 & 21.02 & 21.21 & 20.73\\
    & TransFuse ~\cite{zhang2021transfuse} & 09.05 & 05.75 & 06.58 & 07.15 & 06.25 & 06.96 \\
    & SSFormer ~\cite{wang2022stepwise} & 22.65 & 17.67 & 16.57 & 17.95 & 16.02 & 18.17\\
    & Swin-UNet \cite{cao2022swin} & 05.03 & 02.38 & 02.32 & 05.08 & 04.16 & 03.79\\
    & SAM ~\cite{kirillov2023segment} & 02.14 & 02.11 & 00.77 & 00.73 & 01.62 & 01.47\\
    & SAM (box) ~\cite{kirillov2023segment} & 02.09 & 01.45 & 01.34 & 01.40 & 01.31 & 01.52\\
    & SAM (point) ~\cite{kirillov2023segment} & 06.86 & 04.49 & 03.10 & 02.65 & 04.85 & 04.39\\
    & MedSAM ~\cite{ma2023segment} & 02.13 & 01.71 & 01.66 & 01.49 & 01.64 & 01.73\\
    & \textbf{EFCNet(Ours)} & \textbf{35.06} & \textbf{31.45} & \textbf{29.84} & \textbf{29.35} & \textbf{30.25} & \textbf{31.19}\\			
    \bottomrule
  \end{tabular}
\end{table}

\begin{table} \small
  \caption{Comparison of our EFCNet with competitors  on S-Polyp in DSC ($\%$) and IoU ($\%$).}
  \label{all_clinicdb}
  \centering
  \tabcolsep=0.05cm
  \begin{tabular}{cccccccc}
    \toprule
    Metrics & Methods & Fold0 & Fold1 & Fold2 & Fold3 & Fold4 & Mean \\
    \midrule
    \multirow{14}*{DSC ($\%$)} 
    & U-Net \cite{ronneberger2015u} & 75.90 & 75.47 & 81.95 & 72.06 & 76.73 & 76.42\\
    & U-Net-Large ~\cite{ronneberger2015u} & 78.93 & 78.32 & 82.76 & 73.70 & 77.84 & 78.31\\
    & Attn-UNet ~\cite{oktay2018attention} & 79.89 & 81.17 & 81.19 & 77.01 & 74.68 & 78.79\\
    & MSU-Net ~\cite{su2021msu} & 88.61 & 87.63 & 87.13 & 83.99 & 76.46 & 84.76\\
    & CaraNet \cite{lou2022caranet} & 85.12 & 78.66 & 88.14 & 75.02 & 82.56 & 81.90\\
    & TransUNet \cite{chen2021transunet} & 84.83 & 82.13 & 88.24 & 76.53 & 82.85 & 82.92\\
    & TransFuse \cite{zhang2021transfuse} & 80.73 & 72.43 & 82.33 & 72.53 & 81.04 & 77.81\\
    & SSFormer \cite{wang2022stepwise} & 85.92 & 84.44 & 88.00 & 78.80 & 83.37 & 84.11\\
    & Swin-UNet \cite{cao2022swin} & 48.16 & 53.91 & 50.00 & 49.57 & 61.68 & 52.66\\
    & SAM \cite{kirillov2023segment} & 44.65 & 40.57 & 49.94 & 56.43 & 46.31 & 47.58\\
    & SAM (box) \cite{kirillov2023segment} & 77.21 & 80.40 & 82.65 & 77.73 & 78.60 & 79.32\\
    & SAM (point) \cite{kirillov2023segment} & 72.53 & 73.27 & 75.30 & 67.80 & 72.08 & 72.20\\
    & MedSAM ~\cite{ma2023segment} & 76.46 & 79.26 & 80.97 & 75.26 & 78.70 & 78.13\\
    & \textbf{EFCNet(Ours)} & \textbf{89.11} & \textbf{90.74} & \textbf{89.20} & \textbf{85.39} & \textbf{83.58} & \textbf{87.60}\\
    \midrule
    \multirow{14}*{IoU ($\%$)} 
    & U-Net \cite{ronneberger2015u} & 65.98 & 68.77 & 73.42 & 63.67 & 58.63 & 66.09\\
    & U-Net-Large \cite{ronneberger2015u} & 68.93 & 69.99 & 76.75 & 65.98 & 62.55 & 69.84\\
    & Attn-UNet ~\cite{oktay2018attention} & 72.69 & 72.59 & 73.30 & 68.58 & 68.38 & 71.12\\
    & MSU-Net ~\cite{su2021msu} & 81.50 & 80.80 & 79.34 & 74.92 & 70.21 & 77.35\\
    & CaraNet \cite{lou2022caranet} & 77.24 & 72.04 & 81.40 & 67.29 & 75.56 & 74.71\\
    & TransUNet \cite{chen2021transunet} & 75.40 & 75.29 & 81.02 & 68.83 & 75.20 & 75.15\\
    & TransFuse \cite{zhang2021transfuse} & 70.77 & 64.74 & 74.47 & 65.13 & 73.01 & 69.62\\
    & SSFormer \cite{wang2022stepwise} & 77.16 & 76.30 & 79.93 & 70.74 & 75.52 & 75.93\\
    & Swin-UNet ~\cite{cao2022swin}& 37.36 & 41.84 & 39.23 & 38.00 & 50.10 & 41.31\\
    & SAM \cite{kirillov2023segment} & 39.17 & 35.44 & 44.97 & 51.01 & 41.50 & 42.42\\
    & SAM (box) \cite{kirillov2023segment} & 67.04 & 70.62 & 72.97 & 67.71 & 69.34 & 69.54\\
    & SAM (point) \cite{kirillov2023segment} & 64.17 & 65.89 & 67.54 & 60.15 & 65.60 & 64.67\\
    & MedSAM ~\cite{ma2023segment} & 66.47 & 69.21 & 71.61 & 65.59 & 69.13 & 68.40\\
    & \textbf{EFCNet(Ours)} & \textbf{82.54} & \textbf{83.71} & \textbf{82.08} & \textbf{76.98} & \textbf{75.59} & \textbf{80.18}\\			
    \bottomrule
  \end{tabular}
\end{table}

\begin{table} \small
  \caption{Model cost comparison of our EFCNet with previous methods.}
  \label{modelcost}
  \centering
  \begin{tabular}{cccc}
    \toprule
    Structures & Methods & Flops (G) & Params (M)\\
    \midrule
    \multirow{5}*{CNN}
    & U-Net \cite{ronneberger2015u} & 128.49 & 37.66\\
    & U-Net-Large \cite{ronneberger2015u}& 487.12 & 100.37\\
    & Attn-UNet ~\cite{oktay2018attention} & 125.98 & 34.88\\
    & MSU-Net ~\cite{su2021msu} & 147.10 & 47.09\\
    & CaraNet \cite{lou2022caranet} & 65.25 & 44.59\\
    \midrule
    \multirow{4}*{Transformer}
    & TransUnet \cite{chen2021transunet} & 60.98 & 93.23\\
    & TransFuse \cite{zhang2021transfuse} & 62.10 & 143.39\\
    & SSFormer \cite{wang2022stepwise}& 68.43 & 26.85\\
    & Swin-Unet ~\cite{cao2022swin}& 8.69 & 41.34\\
    \midrule
    \multirow{3}*{Ours}
    & U-Net+CSAA & 466.92 & 87.37\\
    & U-Net+MPS & 138.03 & 38.81\\
    & EFCNet & 476.45 & 88.52\\
    \bottomrule
  \end{tabular}
\end{table}


As shown in Tab.~\ref{all_hrd} and Tab.~\ref{all_clinicdb}, our model achieves the best performance in all folds  on both S-HRD and S-Polyp in terms of DSC and IoU, compared to previous SOTA models.

On S-HRD, our model improves by 6.52$\%$ in terms of DSC and 5.56$\%$ in terms of IoU compared with the previous methods. On S-Polyp, our model improves by 3.49$\%$ according to DSC and 4.25$\%$ according to IoU.

It can be seen that all methods tend to perform poorly on S-HRD. That is because the objects in S-HRD are smaller in size compared with S-Polyp, which means that there is less information available in images. Nevertheless, our model still performs best among all methods. Our CSAA module and MPS module effectively reduce the information loss of small medical objects in the encoder and decoder respectively, thereby enhancing the segmentation ability of our model. 

Moreover, through the experimental results on S-HRD and S-Polyp, it can be found that the smaller the medical objects in datasets, the higher the improvement of our model compared with other methods, which demonstrates the superiority of our model in small medical objects segmentation.

In addition, we compare the cost of the different models in Tab.~\ref{modelcost}. As can be seen, simply increasing the size of U-Net (U-Net-Large) only has a slight improvement in segmentation performance compared to the normal size U-Net, while our EFCNet has a large improvement. This proves that the superior performance of our EFCNet on segmentation is mainly due to our model design rather than the larger model size. Although the addition of CSAA and MPS will increase the costs of the model, we believe that the cost is acceptable, given the significant improvement of our method in the field of small medical object segmentation.

\subsection{Visualization}

\begin{figure*}
    \centering
    \includegraphics[width=14cm]{sota_final.pdf}
    \caption{Visualization of EFCNet (ours) and previous SOTA methods on S-HRD and S-Polyp.}
    \label{v_all}
\end{figure*}

Some visual results of different methods on S-HRD and S-Polyp are shown in Fig.~\ref{v_all}. Compared with other methods, the advantages of our method are mainly reflected in two aspects: segmenting local details such as the boundary of lesion, and capturing extremely small medical objects such as some tiny dots in S-HRD whose area is less than 20 pixels. 

On the one hand, CSAA helps our model apply useful local information contained in low-level features of the encoder to the segmentation procedure, ensuring the segmentation ability for fine details of small medical objects. On the other hand, MPS helps our model take advantage of the global perception contained in low-resolution features in the first few stages of the decoder, improving the ability of our model to locate small objects.

Compared to our model, previous methods are prone to failure in the segmentation of local details and extremely small medical objects.

\subsection{Ablation Studies}

\begin{table} \small
  \caption{Ablation study on CSAA module and MPS module on S-HRD and S-Polyp in DSC ($\%$) and IoU ($\%$).}
  \label{abla_all}
  \centering
  \tabcolsep=0.03cm
  \begin{tabular}{ccccc}
    \toprule
    \multirow{2}*{Methods} & \multicolumn{2}{c}{S-HRD} & \multicolumn{2}{c}{S-Polyp} \\
    & DSC ($\%$) & IoU ($\%$) & DSC ($\%$) & IoU ($\%$)\\
    \midrule
    U-Net & 36.58 & 24.14 & 69.98 & 63.27\\
    U-Net+CSAA & 39.19 & 27.09 & 78.84 & 70.66\\
    U-Net+MPS & 38.98 & 26.85 & 80.20 & 74.14\\
    \textbf{Unet+CSAA+MPS (Ours)} & \textbf{41.82} & \textbf{29.69} & \textbf{83.26} & \textbf{76.29}\\		
    \bottomrule
  \end{tabular}
\end{table}


We perform several sets of ablation experiments on S-HRD and S-Polyp, confirming the positive effect of CSAA and MPS on segmentation ability for small medical objects respectively.

\noindent \textbf{Effectiveness of CSAA and MPS}.
We add CSAA and MPS to our U-Net backbone respectively, and the experimental results are shown in the Tab.~\ref{abla_all}. It can be seen that each module helps our model improve its performance. Moreover, after adding both CSAA and MPS, the segmentation ability of our model can be further improved.

\begin{table} \small
  \caption{Ablation study on the number of stages that CSAA aggregates on S-HRD and S-Polyp in DSC ($\%$) and IoU ($\%$).}
  \label{abla_csaa}
  \centering
  \tabcolsep=0.05cm
  \begin{tabular}{ccccc}
    \toprule
    \multirow{2}*{Methods} & \multicolumn{2}{c}{S-HRD} & \multicolumn{2}{c}{S-Polyp} \\ 
    & DSC ($\%$) & IoU ($\%$) & DSC ($\%$) & IoU ($\%$)\\
    \midrule
    Concat-One & 38.98 & 26.85 & 80.20 & 74.14\\
    AA-One & 40.37 & 28.13 & 82.36 & 75.94\\
    \textbf{AA-All (Ours)} & \textbf{41.82} & \textbf{29.69} & \textbf{83.26} & \textbf{76.29}\\	
    \bottomrule
  \end{tabular}
\end{table}

\noindent \textbf{Number of Stages in CSAA}.
We change the number of stages aggregated in CSAA module: AA-All aggregates features in all stages of the encoder, which is exactly the CSAA applied in our final model. AA-One only performs axial attention on features in one stage of the encoder. Concat-One only concatenates features in each stage of the encoder to the corresponding decoder without any other processing. The performance of these three methods on S-HRD and S-Polyp is shown in Tab. ~\ref{abla_csaa}. It can be seen that among the three models, Concat-One performs the worst. Compared with Concat-One, AA-One can improve the segmentation ability of the model. CSAA aggregates features of all stages of the encoder and performs best among these three methods above. 


\begin{table} \small
  \caption{Ablation study on the number of MPS connected to the decoder on S-HRD and S-Polyp in DSC ($\%$) and IoU ($\%$).}
  \label{abla_mps}
  \centering
  \tabcolsep=0.05cm
  \begin{tabular}{ccccc}
    \toprule
    \multirow{2}*{Methods} & \multicolumn{2}{c}{S-HRD} & \multicolumn{2}{c}{S-Polyp} \\
    & DSC ($\%$) & IoU ($\%$) & DSC ($\%$) & IoU ($\%$)\\
    \midrule
    MPS-1 & 39.19 & 27.09 & 78.84 & 70.66\\
    MPS-2 & 40.07 & 27.17 & 82.00 & 73.87\\
    MPS-3 & 40.18 & 28.32 & 82.51 & 75.13\\
    \textbf{MPS-4 (Ours)} & \textbf{41.82} & \textbf{29.69} & \textbf{83.26} & \textbf{76.29}\\
    \bottomrule
  \end{tabular}
\end{table}

\noindent \textbf{Number of Supervisions in MPS}.
We change the number of supervisions in the MPS: MPS-4 connects segmentation heads to all stages of the decoder, which is exactly the MPS in our final model. MPS-3, MPS-2, and MPS-1 connect three, two and one segmentation heads to the decoder respectively. The performance of these four models on S-HRD and S-Polyp is shown in Tab.~\ref{abla_mps}. It can be seen that among these four models, the more supervision, the better the performance of the model.


==> sec/4_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/5_conclusion.tex <==
\section{Conclusion}
We propose a novel model called EFCNet to address the challenging task of small object segmentation in medical images. EFCNet pays sufficient attention to all features of each stage in the model, effectively reducing the information loss of small medical objects and improving the segmentation accuracy. Specifically, we propose Cross-Stage Axial Attention Module (CSAA) and Multi-Precision Supervision Module (MPS), which reduce the loss of information in the encoder and decoder respectively, thereby significantly improving the performance of the model. Moreover, we build a new benchmark for small object segmentation research. Our experiment on two datasets demonstrates that CSAA and MPS can help the model improve the accuracy of segmentation, and that our model significantly outperforms previous state-of-the-art models.

\noindent \textbf{Limitations}.
We observe that our model may mistake background noise for small medical objects, which can bring additional error in segmentation. One possible reason is that while our model protects sufficient information about small medical objects, it also preserves a small amount of irrelevant information, which may interfere with the segmentation process. This problem will be left to solve in our future work.


==> sec/intro_his.tex <==


Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

